An Analysis of Mixed Initiative and Collaboration in Information-Seeking Dialogues

The ability to engage in mixed-initiative interaction is one of the core requirements for a conversational search system. How to achieve this is poorly understood. We propose a set of unsupervised metrics, termed ConversationShape, that highlights the role each of the conversation participants plays by comparing the distribution of vocabulary and utterance types. Using ConversationShape as a lens, we take a closer look at several conversational search datasets and compare them with other dialogue datasets to better understand the types of dialogue interaction they represent, either driven by the information seeker or the assistant. We discover that deviations from the ConversationShape of a human-human dialogue of the same type is predictive of the quality of a human-machine dialogue.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> drafts.tex <==
% Research questions:
% (1) What is the structure of an information-seeking dialogue?
%     * how is initiative mixed?
%     * how is user revealment achieved?
%     * how is system revealment achieved?
% (2) what are different types of information-seeking dialogues and what is the difference in structure across these types?
%     * how the structure of asynchronous dialogues (QA forum threads) differ from synchronous dialogues (text chat and audio)?
%     * how chit-chat and task-oriented dialogues are different from other information-seeking dialogues?
% (3) Can we detect it automatically? How to scale this type of conversation analysis?

% how do we evaluate dialogues?

    % Last but not least we set out to examine
    % * how the structure of successful dialogues differ from unsuccessful ones?
    
    % since none of them is annotated with conversation success
    % also the most common failure is not relevant response which is most common for machine-human dialogues but not as common for human-human dialogues
    
    % * how the sructure of human-human dialogues is different from machine-human dialogues?
    
    % we use conversational logs of the SlugBot~\cite{DBLP:conf/cui/BowdenWCJHSSWW19} to answer these questions.
    % SlugBot is one of the participant systems in all Alexa Prize challenges\footnote{\url{https://developer.amazon.com/alexaprize}}.
    % Qualitative evaluation of the SlugBot has already indicated that the system is talking too much without the ability to listen to their user information needs~\cite{DBLP:conf/cui/BowdenWCJHSSWW19}.
    % We conduct an automated evaluation on all conversation logs to discover patterns that lead to conversation failures.
    
    
    % % TODO summarise all RQs
    % Thus, in this paper we dive into conversation analysis of existing conversational datasets to understand structural differences between conversations and detect structural patterns that signal breakdown.
    
    
    

% Another reason is also since it is overlapping with other subfields of Computer Science, such as natural language processing, conversational AI and dialogue systems
% systems open not grounded or grounded but in very restricted domains

    % clearly only one side of conversational search those are focusing on subtasks while the conversational system should support both tasks and be able to combine them in a dialogue
    % the structure is known
    
    % % identify evaluation gaps
    % focus on information-seeking conversations that include both questions and answers
    
    we take one of these datasets (\textbf{MSDialog}~\cite{InforSeek_Response_Ranking}) to examine how its structure differs from other information-seeking dialogues
    
    
  % However this set of properties triggers more questions: 
% neither ground in empirical evidence nor concrete recipes on how this can be achieved. evaluation
% but how?


% motivation


% the most straightforward extension from classic QA and recommendation tasks into conversational settings.
% but how?

% conversational search is complex, i.e. requires different components and interaction types
% one factors that researchers manage to agree upon is that conversational search systems should be sufficiently robust to support different kinds of interactions~\cite{radlinski2017theoretical,vakulenko2019qrfa,penha2019introducing,azzopardi2018conceptualizing}
% in practice often several modules different data sources web search structured knowledge data access across different databases domains with a diverse schema~\cite{rastogi2019scaling}


% Conversational search tasks: information need elicitation and information presentation~\cite{penha2019introducing}


% assuming relevance
% relevant response
   

% (1) What is the structure of an information-seeking dialogue?
%     * how is initiative mixed?
%     * how is user revealment achieved?
%     * how is system revealment achieved?




the structure is known
we use one of this datasets (\textbf{CCPE}~\cite{radlinski2019coached}) to evaluate our utterance classification approach

longer utterances and shorter dialogues. we take one of these datasets (\textbf{MSDialog}~\cite{InforSeek_Response_Ranking}) to examine how its structure differs from other information-seeking dialogues



% Another reason is also since it is overlapping with other subfields of Computer Science, such as natural language processing, conversational AI and dialogue systems
Conversational search has come to distinguish itself from other system types such as chit-chat and task-oriented dialogue systems.
% systems open not grounded or grounded but in very restricted domains

evaluation slugbot


% none of the datasets dialogues annotated with conversation success


 However we also identify gaps where more data is needed.

% (5) What kind of data do we need and why?
%     % that's a give-away!
%     -> we need to have dialogues annotated with conversation success or break-down labels for evaluation
collaboration Delft Claudia 


evaluation challenge an output of a conversational search system is a dialogue given a dialogue decide on success
% either compare to existing dialogues or ask users
but what about strategy can we say that the dialogues that tend to have more mixed initiative tend to be more successful as well because they engage with the seeker
is the conversation system actually listening to the user or acts upon its predefined scenario?
is the system able to understand the information need in a conversation and follow up in the correct direction?
what if there are no predefined intents or slots to do this?
can we measure engagement through vocabulary reuse that can in turn predict user satisfaction?

SCS

% unfortunately how to use a search interface in a scenario rather than a conversational search system e.g. question answer result page analysis and document access however we show exploratory properties such as query refinement exploratory tasks when there is no one single answer requires overview result summary and navigation components

==> model-diagnostics.tex <==

\section{Model Diagnostics}
\label{sec:diagnostics}
% setup description
We show that ConversationShape can be \mdr{``also'' -- what was the  application you mentioned before this point?} also applied to evaluate dialogue models and understand the type of deviant behaviour the model exhibits.
% In this section we report on the experiments using ConversationShape for ranking dialogue models.
These experiments were performed on the subsets of the Control-M dataset that correspond to the transcripts produced by different dialogue models.
There are in total 28 models and we produce a ConversationShape profile for each of them.
Then, we measure cross-entropy between the models' distributions and the distribution calculated for the subset of human-human dialogues (Control-H).
Finally, we compare our results with the human evaluation results reported in the original paper~\cite{see2019what}.
The model with the lowest cross-entropy (0.01) to the human-human distributions was also the model that was preferred by human judges with respect to Interestingness and characterised by better flow and more information sharing.
Moreover, ConversationShape also allows to interpret the type of deviation the model exhibit by observing each of the dimensions separately.
We discovered three types of deviant behavior among the dialogue models in the Control-M dataset:
\begin{itemize}[leftmargin=*,nosep]
    \item \textit{interviewer} -- asking too many questions (three times more often than in Control-H) characterised by high \emph{Question} dimension (correlates with very high values of Inquisitiveness in human judgements).
    \item \textit{talker} -- producing too many unique tokens (optimised for diversity) characterised by high \emph{Information} but low \emph{Repetition} dimensions (correlates with low values for Listening, Interestingness, Inquisitiveness and Sense-making in human judgements).
    \item \textit{parrot} -- producing too few unique tokens (optimised for responsiveness) characterised by low \emph{Information} and high \emph{Repetition} dimensions (correlates with low values for Listening, Interestingness, Inquisitiveness and Sense-making in human judgements).
\end{itemize}

% Using $Questions$ dimension allows to distill models that abuse questioning behaviour.
% We inspect the transcripts of the model that is very skewed towards questioning behaviour and confirm that it indeed asks a question at every turn, which is three times more often than in an average human conversation, often also leaving the questions of the conversation partner unanswered.
% \todo{describe failing models with feature values}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./figs/control.png}
  \caption{Model types in the Control dataset estimated by $Question$ and $Flow$ metrics.}
\end{figure}


==> rel_work.tex <==
\section{Related Work}
\label{sec:rel_work}

This section provides an overview of approaches used for dialogue evaluation demonstrating the lack of research on measuring initiative and collaboration in dialogue.
We also pinpoint the relation of our work to the earlier line of research on mixed-initiative systems, which stems from the discourse analysis approaches proposed in the late 1980th.

\subsection{Dialogue Evaluation Metrics}
The most popular metric for dialogue evaluation is relevance of the response, which is usually measured with respect to the ground-truth response.
It is comparable to the answer accuracy if the response is an answer.
Dialogue responses usually consist of natural language utterances and they are compared to the ground-truth responses using n-gram overlap metrics, such as BLEU, METEOR, and ROUGE~\cite{DBLP:conf/emnlp/LiuLSNCP16}, or cosine similarity between their embeddings~\cite{DBLP:conf/aaai/TaoMZY18}.
Since there can be multiple correct responses, which are not all covered by the ground truth, this metric is rather limited in its application.
% More recent research reports model's perplexity to have high correlation with a human judgement.

Simple automated measures based on discourse features, such as lexical and syntactic diversity, were successfully adopted for training and evaluation of dialogue systems to reduce repetitive generic responses and estimate question complexity~\cite{see2019what,DBLP:journals/corr/abs-1911-03860,DBLP:conf/conversations/JalotaTMNU19}.
We propose to extend unsupervised approaches that compare distributions of lexical features, which were previously used for language style matching~\cite{ireland2010language} and measuring quality of generated narratives~\cite{DBLP:journals/corr/abs-1909-10705}, to a dialogue setting.
The main characteristic of dialogue as a type of narrative is the distribution of utterances between the dialogue participants.
Therefore, we estimate lexical features separately for each participant to be able to compare their contributions and deduce the roles they play in the conversation.

\subsection{Mixed-Initiative Systems}
The most similar to ours is the early work by \citet{DBLP:conf/acl/WalkerW90}, who studied lexical cues, such as the use of anaphors and different utterance types, as the mechanism for switching control across two dialogue types.
\citeauthor{DBLP:conf/acl/WalkerW90}'s study was based on the approach to utterance type classification and the rules for transfer of control between participants proposed by \citet{whittaker1988cues}, which is considered to be the earliest investigation into initiative and design of mixed-initiative dialogue systems.
Allocation of control, where control is defined as the management of the direction of flow in a conversation, is at the core of mixed-initiative dialogue systems that are designed to enhance human-machine collaboration~\cite{Cohen1998}.

Dialogue systems should be able to recognize the user’s cues for initiative switch to provide appropriate responses~\cite{DBLP:journals/umuai/Chu-CarrollB98}.
Detecting initiative is important to characterize the quality of the interaction~\cite{Cohen1998}.
We follow the same hypothesis expressed in earlier work on mixed-initiative dialogue systems that
a set of linguistic cues is sufficient to predict initiative holders from dialogue transcripts~\cite{DBLP:journals/umuai/Chu-CarrollB98}.
Our approach to dialogue representation is domain-independent and allows us to scale such analysis, which was performed only on a handful of dialogues before, to thousands of publicly available dialogue transcripts. 

==> scrap.tex <==

% takes a pair of the dimensions
% , identify similarities and differences, and group them accordingly using different dimensions.
% , e.g. in the majority of the datasets questions are asked mostly by the Seeker.
% The main outliers are CCPE (most questions are asked by Assistant), MultiWOZ (information is provided by the Seeker and repeated by the Assistant) and MSDialog (high Information and Repetition since messages are long and conversations are short).
% outliers ccpe multiwoz forum



In particular, forum threads, which are a popular source for conversational search datasets due to to their availability~\cite{penha2019introducing}, are rather different type of interaction from synchronous dialogues, which limits their application for development of conversational search systems.
On the other hand, common ``chit-chat'' dialogues often exhibit properties similar to information-seeking dialogues, in terms of question-answering, initiative and collaboration, which makes them more suitable candidates for studying patterns characteristic of a human dialogue.


% dataset types plot figure 1 table 1



% closer to the center more assymetric

% human chit chat very similar
% meena is similar to daily

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{./figs/information.png}
%   \caption{Dataset types organised by the number of frequent tokens introduced and the distribution between the roles (more tokens introduced by Assistant on the right, by Seeker -- on the left), i.e., $\Delta Information$ on x-axis and $Information$ on y-axis.}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{./figs/followup.png}
%   \caption{Dataset types organised by the number of reused tokens and the distribution between the roles (more tokens reused by Assistant on the right, by Seeker -- on the left), i.e., $\Delta Follow$-$up$ on x-axis and $Follow$-$up$ on y-axis.}
% \end{figure}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{./figs/4.pdf}
%   \caption{}
% \end{figure*}

    % Table~\ref{tab:datasets} shows means and standard deviations calculated for each metrics over all dialogues in the respective dataset.
    % Each metric was normalised by the number of utterances in the dialogue to better compare dialogues of different length.
    
    % % \todo{describe the scale from the top}
    % In the first three rows of the table are the datasets, in which the Assistant takes over the initiative by asking questions.
    % CCPE dataset was designed as a question-answering dataset and the ConversationShape metrics correctly reflects this property, which is characterised by the high number of questions (0.16 questions per utterance mostly by the Assistant).
    % ReDial has similar properties in terms of role distribution, but is much more balanced.
    % Assistant in ReDial also contributes more frequent tokens to the discussion rather than just consuming information from the Seeker as in CCPE.
    
    % MultiWOZ is very distinct from all other datasets since Assistant holds the initiative across all the dimensions except for Information.
    % This indicates a kind of browsing interaction where Assistant constantly requests information and immediately follows up, while the role of the Seeker is to determine the direction of the exploration by answering the questions.
    
    % % Almost all questions were asked by the Assistant ()
    % % \todo{last two machine dialogues to show deviation in the next section compare models}
    % % , e.g.
    
    % The rest of the datasets are driven by Seeker asking questions rather then Assistant as in the first three ($\Delta Question$).
    % Notice that CCPE and SCS are symmetric with respect to the $\Delta$ features.
    % This shows that SCS is structurally similar to CCPE but with the roles swapped.
    % Most of the information is to be provided by the Assistant and the Seeker defines direction of the search by asking follow-up questions.
    % Notice, also the difference in the average number of repetitions, which is higher for MultiWOZ, SCS and WoW, while lower for CCPE and ReDial.
    % This metric correlates with the focus of the discussion on a specific topic, such as a specific information need in SCS, or a more general and broad topic discussion, such as movie preferences in CCPE and ReDial.
    
    % Note, how not only WoW but also DailyDialog, which is considered to be a chit-chat dialogue corpus, both follow the same distribution as SCS.
    % MSDialog is one of the major outliers.
    % Due to the nature of the asynchronous interaction medium (an on-line forum) the conversations are shorter and the utterances are much longer, which makes them appear much more dense than all other dialogue datasets.
    
    % % In both cases one of the partner is mainly asking the questions ($\Delta Question$) and the other partner is mainly replying ($\Delta Length$, $\Delta Repeat$, $\Delta Anaphora$).
    % % It is worth noting that the average number of questions per utterance is much higher for CCPE and the repetitions are less than in SCS.
    % % These measures indicate that SCS is mostly focused on information elicitation like CCPE but is more focused since the scope of conversation is on a single search topic, while in CCPE many different topics related to movies are discussed.
    % % This way we separate two dimensions that correlate with our features: (1) question answering (QuestionA) and (2) topic breadth (RepeatA). 
    
    % % Now using these dimensions we identify other datasets that are similar, e.g. MultiWOZ has a higher number of questions and repetitions than SCS, but the questions are asked mostly by Provider and the utterance length is twice shorter.
    % % % MSDialog is the major outliers in terms of utterance length, which shows also in increased number of repetition and anaphora use.
    % % % It also contain less turns per dialogue than other datasets.
    % % The question distribution in MSDialog is more balanced than in CCPE and SCS as well as the utterance length.
    % % The utterances in MSDialog are much longer, which shows also in increased number of repetition and anaphors.
    
    % % ReDial is one of only three datasets where questioning is dominated by the Information Provider.
    % % It is similar to CCPE but much more balanced in terms of length and repetition distributions.
    % % WoW is similar to SCS in terms of question distribution but more equally distributed in terms of repetitons and utterance length.
    
    % % The last four datasets are typical examples of chit-chat dialogues.
    % % Interesting that these dialogues also show a high degree of question-answering interactions.
    % % In DailyDialogues there are no annotated roles but questioning is mostly skewed  towards the participant starting the conversation, which we, therefore, assigned the role of Information Seeker.
    % % The use of anaphors and utterance lengths are balanced but repeat and question patterns indicate that one of the conversation participants is leading the conversation.
    
    % The last two rows show results for machine-human dialogues.
    % There is a clear difference between the distributions of machine-human and human-human dialogues.
    % Both Control-M and ConvAI2 receives the smallest scores on the $Follow$-$up$ metric.
    % They are also more imbalanced on all $\Delta$ metrics except for $\Delta Follows$.
% There is also a very large discrepancy between utterance lengths in ConvAI2 dataset, which again suggests that users did not engage with the chatbots often responding with short utterances.

% The abnormally low degree of repetitions also signals that there is no engagement between the participants reflected in the absence of shared vocabulary.
% Both datasets also reflect incompetence of dialogue models in using anaphors.
% Control dataset has a 
% and number of turns per dialogue
% , which indicates various dimensions of initiative and highlights similarities between dialogue types.% 
